Towards Consistency in Adversarial Classification

In this paper, we study the problem of consistency in the context of adversarial examples. Specifically, we tackle the following question: can surrogate losses still be used as a proxy for minimizing the $0/1$ loss in the presence of an adversary that alters the inputs at test-time? Different from the standard classification task, this question cannot be reduced to a point-wise minimization problem, and calibration needs not to be sufficient to ensure consistency. In this paper, we expose some pathological behaviors specific to the adversarial problem, and show that no convex surrogate loss can be consistent or calibrated in this context. It is therefore necessary to design another class of surrogate functions that can be used to solve the adversarial consistency issue. As a first step towards designing such a class, we identify sufficient and necessary conditions for a surrogate loss to be calibrated in both the adversarial and standard settings. Finally, we give some directions for building a class of losses that could be consistent in the adversarial framework.

==> sections/codeofconduct.tex <==
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} The work brings theoretic insights on adversarial robustness. We believe there is no potential social harm in our work.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} Every result is stated with clear hypothesis.
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} All proofs are in Appendix.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> sections/consistencySurrogateConvex.tex <==
\section{Calibration in the Adversarial Setting}

The overwhelming majority of machine learning algorithms use convex surrogate losses, since they are the easier to optimize. 

In this section, we will show that these losses are ill-suited for the adversarial setting : a sequence of function can minimize the surrogate risk while performing arbitrarily bad for the $0-1$ loss.

This is due to a pathological phenomenon that appears in the adversarial setting. For example in Figure \ref{fig:my_label}, classifying $Z_1$ and $Z_2$ both as $1$ or both as $-1$ leads to the optimal $0-1$ risk of $\frac{1}{2}$, whereas classifying them differently leads to a risk of $0$. For any convex surrogate loss, the optimal classifier for this distribution would return $0$ on both zones. Even though that returns the same class at the optimum, a minimizing sequence for the $\phi$-risk may keep $Z_1$ and $Z_2$ classified differently while just lowering the values, thus keeping a risk of $0$ for the $0-1$ loss.

This is formalized in the next proposition :

\begin{prop}
Let $\phi$ be convex, classification-calibrated loss ($\phi'(0) <0$). Then for any $\epsilon > 0$, $\phi$ is not $\epsilon -$adversarially consistent with $l_{0/1}$.
\end{prop}

\begin{prv*}

Let $\epsilon > 0$. We will construct a distribution $\mathcal{D}$ and a sequence of classifier $h_n$ so that the $\phi$-risk converges toward the optimal, while the $0-1$ loss remains constant at a non-optimal value.

\paragraph{}Let a such that $\epsilon < a < 2 \epsilon$. We define D by :
\[
\left\{ \begin{array}{ll}
\mathbb{P}(Y=1, X=0) = \frac{1}{2} & \\
\mathbb{P}(Y=-1, X=-a) = \frac{1}{4} & \\
\mathbb{P}(Y=-1, X=a) = \frac{1}{4} & \\
\mathbb{P}(X=x, Y=y) = 0 & \mbox{for any other (x,y).} \\
\end{array} \right.
\]

Since $\phi$ is classification-calibrated, it is either non-increasing, or it has a minimum, attained on a point $u>0$. Let us consider both cases :

\paragraph{First case : $\phi$ non-increasing}

We define $Z_1 = [-\epsilon, -a + \epsilon]$ and $Z_2 = [a-\epsilon, \epsilon]$, the zones that can be attacked by two points at once.
Let us then define : 
\[
\forall x \in \mathbb{R}, h_n(x) = \left\{ \begin{array}{ll}
\frac{1}{n} & \mbox{if } x \in Z_1 \\
-1/n & \mbox{if } x \in Z_2 \\
1 & \mbox{if }x \in [-a+\epsilon, a-\epsilon] \\
-1 & \mbox{otherwise} \\
\end{array} \right.
\]

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/Exemple.png}
    \caption{The distribution we use as a counter-example. For the $0-1$ loss, there are two optimal classifiers, putting either both $Z_1$ and $Z_2$ to $1$ (and saving point A), or both to $-1$ (saving points B and C). With convex surrogate losses however, the optimal is to bring values in both $Z_1$ and $Z_2$ to zero, which can be done while maintaining opposite signs on $Z_1$ and $Z_2$, and so ensuring the loss of both A and one of B and C for the $0-1$ loss. }
    \label{fig:my_label}
\end{figure}


Since the central point and the point $x=-a$ are attackable, but not the point $x=a$, we have $\mathbb{E}_{(x,y)\sim \mathcal{D}}\left[ \sup\limits_{z \in \mathcal{B}(x,\epsilon)} l_{0/1}(y,h_n(z))\right] = \frac{3}{4}$, which is worse than the constant classifier h=1, which gives a score of $\frac{1}{2}$. So $h_n$ is not a minimizing sequence for the $0-1$ loss.

Let us now show that $h_n$ is a minimizing sequence for the loss $\phi$ under attack, which will be proof of the non-consistency.

\begin{align*}
    \mathbb{E}_{(x,y)\sim \mathcal{D}}\left[ \sup\limits_{z \in \mathcal{B}(x,\epsilon)} \phi(y*h_n(z))\right] &= \frac{1}{2} \phi(\frac{-1}{n}) +\frac{1}{4}\phi(\frac{1}{n}) + \frac{1}{4}\phi(\frac{1}{n})\\
    &=\frac{1}{2}\phi(\frac{-1}{n}) + \frac{1}{2}\phi(\frac{1}{n}) \\
    &\underset{n\to +\infty}{\longrightarrow}\phi(0)
\end{align*}

We now need to show that $\phi(0)$ is a lower bound of the optimal adversarial risk for the loss $\phi$.
Let h be any  classifier. We define :
\begin{align*}
b &= \inf\limits_{z \in \left[ -a + \epsilon, a- \epsilon \right]} h(z) \\
c &= \sup\limits_{z \in \left[ -a - \epsilon, -\epsilon \right]} h(z) \\
d &= \sup\limits_{z \in \left[\epsilon, a + \epsilon \right]} h(z) \\
m_i &= \inf\limits_{z \in \mathcal{Z}_i} h(z) \mbox{  for  }i \in \left\{ 1,2\right\} \\
M_i &= \sup\limits_{z \in \mathcal{Z}_i} h(z) \mbox{  for  }i \in \left\{ 1,2\right\} \\
m &= \min(m_1,m_2)
\end{align*}

We then have :

\begin{align*}
    &\mathbb{E}_{(x,y)\sim \mathcal{D}}\left[ \sup\limits_{z \in \mathcal{B}(x,\epsilon)} \phi(y*h_n(z))\right] \\
    &= \frac{1}{2} \sup\limits_{ z \in \left[ -\epsilon, \epsilon \right]} \phi(h(z))
            + \frac{1}{4}\sup\limits_{z \in \left[ -a-\epsilon, -a+\epsilon \right]} \phi(-h(z)) 
            + \frac{1}{4}\sup\limits_{z \in \left[ a-\epsilon, a+\epsilon \right]} \phi(-h(z)) \\
    &= \frac{1}{2} \max \left[ \sup\limits_{ z \in \left[ -a+\epsilon, a-\epsilon \right]} \phi(h(z)), \sup\limits_{ z \in \mathcal{Z}_1} \phi(h(z)), \sup\limits_{ z \in \mathcal{Z}_2} \phi(h(z)) \right] \\
    &+ \frac{1}{4} \max \left[ \sup\limits_{ z \in \left[ -a-\epsilon, -\epsilon \right]} \phi(-h(z)), \sup\limits_{ z \in \mathcal{Z}_1} \phi(-h(z)) \right] \\
    &+ \frac{1}{4} \max \left[ \sup\limits_{ z \in \left[ \epsilon, a+\epsilon \right]} \phi(-h(z)), \sup\limits_{ z \in \mathcal{Z}_2} \phi(-h(z)) \right] \\
    &= \frac{1}{2} \max \left[ \phi(b), \phi(m_1), \phi(m_2) \right]
    + \frac{1}{4} \max \left[ \phi(-M_1), \phi(-c) \right] \\
    &+ \frac{1}{4} \max \left[ \phi(-M_2), \phi(-c) \right] \\
    &\geq \frac{1}{2} \max \left[\phi(m_1), \phi(m_2) \right] + \frac{1}{4}\phi(-M_1) + \frac{1}{4}\phi(-M_2) \\
    &\geq \frac{1}{2} \phi(m) + \frac{1}{4}\phi(-m) + \frac{1}{4}\phi(-m) \\
    &\geq \phi(0)
\end{align*}

Hence the result.
\end{prv*}




\section{Towards Consistency}

\begin{prop}
Let $\PP$ be a Borel probability distribution over $\mathcal{X}\times\mathcal{Y}$ such that $\mathcal{R}^{\varepsilon}_\PP = 0$. Then, let $\phi$ be a standard classification calibrated margin-based loss. Then $\Tilde{\phi}:(x,y,f)\mapsto\sup_{x'\in B_\varepsilon(x)}\phi(yf(x'))$ is adversarially consistent at level $\varepsilon$.
\end{prop}



\begin{prop}
No convex losses are calibrated
\end{prop}
\begin{prv*}

Let $\PP= \frac{1}{2}\left(\delta_{x=x_1,y=1}+\delta_{x=x_2,y=-1}\right)$ such that $\lVert x_1-x_2\rVert<2\varepsilon$. We have:
$$R_{\phi,\PP}(f) = \frac{1}{2}\left(\sup_{x\in B_\varepsilon(x_1)}\phi(1,f(x))+\sup_{x\in B_\varepsilon(x_2)}\phi(-1,f(x))\right)$$.

Let $a,b$ s.t. $a\neq b$  $\lVert a-x_i\rVert<\varepsilon$ and  $\lVert b-x_i\rVert<\varepsilon$ for $i\in\{1,2\}$ (they exist under mild assumptions on $\mathcal{X}$). We then have: 
\begin{align*}
R^*_{\phi,\PP} & \geq \inf_{f} \frac{1}{2}\Big(\max\left(\phi(1,f(a)),\phi(1,f(b))\right)\\
&+
\max\left(\phi(-1,f(a)),\phi(-1,f(b))\right)\Big)\\
&=  \inf_{\alpha,\beta} \frac{1}{2}\left(\max\left(\phi(1,\alpha),\phi(1,\beta)\right)+\max\left(\phi(-1,\alpha)),\phi(-1,\beta)\right)\right)\\
&:= \inf_{\alpha,\beta} r(\alpha,\beta)
\end{align*}

Let us show it is actually an equality. Let define $f_n$ as follows:
\begin{align*}
    f_n(x) = \left\{
    \begin{array}{ll}
        0 & \mbox{si } \lVert x-x_1\rVert >\varepsilon\mbox{ et } \lVert x-x_2\rVert >\varepsilon\\
        u_n & \mbox{si } \lVert x-x_1\rVert >\varepsilon\mbox{ et } \lVert x-x_2\rVert\leq \varepsilon\\
        v_n & \mbox{si } \lVert x-x_1\rVert \leq\varepsilon\mbox{ et } \lVert x-x_2\rVert> \varepsilon\\
        \alpha_n & \mbox{si } \lVert x-x_1\rVert \leq\varepsilon\mbox{ et } \lVert x-x_2\rVert> \varepsilon\\
        \beta_n & \mbox{si } \lVert x-x_1\rVert \leq\varepsilon\mbox{ et } \lVert x-x_2\rVert> \varepsilon\\
    \end{array}
\right.
\end{align*}
with $\phi(1,u_n)\to \inf_t \phi(1,t)$, $\phi(-1,v_n)\to \inf_t \phi(-1,t)$ and $r(\alpha_n,\beta_n)\to\inf_{\alpha,\beta} r(\alpha,\beta)$. Then one can check that $$R_{\phi,\PP}(f_n)\to \inf_{\alpha,\beta} r(\alpha,\beta)$$. 

The loss being calibrated for standard classification problems, we have: $u_n>0$ and $v_n<0$ for $n$ sufficiently large. Then we have
\begin{align*}
    R_{0/1}(f_n) &= \frac12 \left(\max(\mathbf{1}_{sign(\alpha_n)\leq0},\mathbf{1}_{sign(\beta_n)\leq0})+\max(\mathbf{1}_{sign(\alpha_n)\geq0},\mathbf{1}_{sign(\beta_n)\geq0})\right)\\
    & =\frac12 \left(\mathbf{1}_{\max(\alpha_n,\beta_n)<0}+\mathbf{1}_{\min(\alpha_n,\beta_n)\geq0}\right)
\end{align*}

And of course we have: $R_{0/1}^\star=\frac12$

\textbf{Convex case:} $\phi(1,\cdot)$ and $\phi(-1,\cdot)$ are convex hence $(0,0)$ realizes the minimum of $r$ then one could set $(\alpha_n,\beta_n)=(\frac1n,-\frac1n)$ and we have in this case $R_{0/1}(f_n)=1$ for $n$ sufficienlty large. 
\end{prv*}

